Empowering Reliable Visual-Centric Instruction Following in MLLMs

Evaluating the instruction-following (IF) capabilities of Multimodal Large Language Models (MLLMs) is essential for rigorously assessing how faithfully model outputs adhere to user-specified intentions. Nevertheless, existing benchmarks for evaluating MLLMs' instruction-following capability primarily focus on verbal instructions in the textual modality. These limitations hinder a thorough analysis of instruction-following capabilities, as they overlook the implicit constraints embedded in the semantically rich visual modality. To address this gap, we introduce VC-IFEval, a new benchmark accompanied by a systematically constructed dataset that evaluates MLLMs' instruction-following ability under multimodal settings. Our benchmark systematically incorporates vision-dependent constraints into instruction design, enabling a more rigorous and fine-grained assessment of how well MLLMs align their outputs with both visual input and textual instructions. Furthermore, by fine-tuning MLLMs on our dataset, we achieve substantial gains in visual instruction-following accuracy and adherence. Through extensive evaluation across representative MLLMs, we provide new insights into the strengths and limitations of current models.

==> templates/failure_case_ex.tex <==
\begin{figure*}[h!]
\begin{tcolorbox}[
    colback=blue!1!white,
    colframe=blue!70!black, 
    title=Judgement Failure case,
    colbacktitle=blue!5!white,
    coltitle=blue!50!black,
    fonttitle=\bfseries,
    boxrule=0.5pt,
    arc=4pt,
    boxsep=5pt,
    left=6pt,
    right=6pt,
    top=6pt,
    bottom=6pt,
    coltitle=blue!50!black
]

\textbf{Question: } The concept of congruence is as follows: When dividing integers \(a\) and \(b\) by a given positive integer \(m\), if the remainders (natural numbers less than the positive integer \(m\), i.e., \(0, 1, 2,\cdots, m - 1\)) are equal, then \(a\) and \(b\) are said to be congruent modulo \(m\), denoted as \(a\equiv b(\text{mod}m)\). Two congruence equations with the same modulus can also be added and subtracted. The operation rules are as follows: Given integers \(a\), \(b\), \(c\), \(d\) and a positive integer \(m\), if \(a\equiv b(\text{mod}m)\) and \(c\equiv d(\text{mod}m)\), then \(a + c\equiv b + d(\text{mod}m)\) and \(a - c\equiv b - d(\text{mod}m)\). If \(a = a_{n}\times10^{n}+a_{n - 1}\times10^{n - 1}+\cdots + a_{1}\times10^{1}+a_{0}\times10^{0}\), where \(a_{n}\) is a positive integer and \(n\) is a non - negative integer, prove that \(a\) is divisible by \(11\) if and only if \(a_{0}-a_{1}+a_{2}-a_{3}+\cdots+(-1)^{n}a_{n}\) is divisible by \(11\).

\textbf{Model: }\textit{Deepseek-r1-0120}

\textbf{Failure Mode}: \textit{Incomplete Proof}

\textbf{Answer:} 
To prove that a number \(a\) is divisible by 11 if and only if the alternating sum of its digits \(a_0 - a_1 + a_2 - a_3 + \cdots + (-1)^n a_n\) is divisible by 11, we use properties of modular arithmetic.

1. **Key Congruence**: Note that \(10 \equiv -1 \pmod{11}\). Therefore, \(10^k \equiv (-1)^k \pmod{11}\) for any non-negative integer \(k\).

2. **Expressing \(a\) in Terms of Congruences**:
   - Consider the number \(a = a_n \times 10^n + a_{n-1} \times 10^{n-1} + \cdots + a_1 \times 10 + a_0\).
   - Using the congruence \(10^k \equiv (-1)^k \pmod{11}\), we can rewrite each term modulo 11:
     \[
     a \equiv a_n \times (-1)^n + a_{n-1} \times (-1)^{n-1} + \cdots + a_1 \times (-1) + a_0 \times 1 \pmod{11}
     \]

3. **Simplifying the Expression**:
   - This simplifies to the alternating sum of the digits:
     \[
     a \equiv a_0 - a_1 + a_2 - a_3 + \cdots + (-1)^n a_n \pmod{11}
     \]

4. **Conclusion**:
   - Therefore, \(a \equiv 0 \pmod{11}\) if and only if the alternating sum \(a_0 - a_1 + a_2 - a_3 + \cdots + (-1)^n a_n \equiv 0 \pmod{11}\).

This proves both directions of the statement: \(a\) is divisible by 11 if and only if the alternating sum of its digits is divisible by 11.

\textbf{Judge Model: }\textit{Gemini2.5-Pro-Preview-0506}

\textbf{Judgement: }
The main issue concerns the justification for the properties used in steps 1 and 2. The problem statement provides:
(D) The definition of congruence: \(a \equiv b \pmod m\) if \(a\) and \(b\) have the same remainder when divided by \(m\).
(R) Operation rules: If \(a \equiv b \pmod m\) and \(c \equiv d \pmod m\), then \(a+c \equiv b+d \pmod m\) and \(a-c \equiv b-d \pmod m\).

The proof relies on:
(P1) If \(x \equiv y \pmod m\), then \(x^k \equiv y^k \pmod m\). (Used for \(10^k \equiv (-1)^k\)).
(P2) If \(x \equiv y \pmod m\), then \(c x \equiv c y \pmod m\). (Used for \(a_i 10^i \equiv a_i (-1)^i\)).

These properties (P1 and P2) are not explicitly listed in the provided "operation rules". While they are standard results in modular arithmetic and can be derived from the given definition (D), the student uses them without derivation.Using (P1) and (P2) without derivation or justification from the given rules/definition constitutes a "Incomplete Proof." The argument's logic is sound if these properties are assumed, but their use is not directly justified by the problem's setup.
\end{tcolorbox}
\caption{An example here.}
\label{fig:judge-1}
\end{figure*}
